Modeling Collaborator: Enabling Subjective Vision Classification With Minimal Human Effort via LLM Tool-Use

From content moderation to wildlife conservation, the number of applications that require models to recognize nuanced or subjective visual concepts is growing. Traditionally, developing classifiers for such concepts requires substantial manual effort measured in hours, days, or even months to identify and annotate data needed for training. Even with recently proposed Agile Modeling techniques, which enable rapid bootstrapping of image classifiers, users are still required to spend 30 minutes or more of monotonous, repetitive data labeling just to train a single classifier. Drawing on Fiske's Cognitive Miser theory, we propose a new framework that alleviates manual effort by replacing human labeling with natural language interactions, reducing the total effort required to define a concept by an order of magnitude: from labeling 2,000 images to only 100 plus some natural language interactions. Our framework leverages recent advances in foundation models, both large language models and vision-language models, to carve out the concept space through conversation and by automatically labeling training data points. Most importantly, our framework eliminates the need for crowd-sourced annotations. Moreover, our framework ultimately produces lightweight classification models that are deployable in cost-sensitive scenarios. Across 15 subjective concepts and across 2 public image classification datasets, our trained models outperform traditional Agile Modeling as well as state-of-the-art zero-shot classification models like ALIGN, CLIP, CuPL, and large visual question-answering models like PaLI-X.

==> old/abstract_v1.tex <==
Modeling Copilot is an orchestration of large language models (LLMs) and vision-language models (VLMs) that aims at solving a variety of visual tasks. We focus on the Agile Modeling task on nuanced visual concepts. Classical modeling systems require human effort from both users and crowd annotators for classification. In our system, we aim to reduce human effort and bias, and scale up data mining and annotation in the Agile modeling system, leveraging different degrees of autonomy. Our system is prompted using a concept name and its description, and using LLMs with tool-use, we output a light-weight distilled binary classifier. We utilize visual query answering models (i.e., PaLI) as tools to the supervisor LLM that asks relevant questions about a given image and aggregates the answers of those questions using logical reasoning to make a final prediction. We measure the success of or system on Agile Modeling nuanced concepts as well as a selection of mainstream image classification sets. We show that our Modeling Copilot system is on par with Agile Modeling, achieving similar classification performance with zero human effort. Additionally, we show that our method exceeds the performance of zero-shot classification models like CLIP and PaLI.
%First, we use an LLM to structure the input concept definition into in-scope (positive) attributes and out-of-scope (negative) attributes. We further use LLMs to generate atomic questions regarding the concept which a visual-question-answering (VQA) model (i.e. PaLI) can answer. For a given image, we aggregate questions and answers generated by this process and leverage the LLMs chain-of-thoughts reasoning capabilities to draw a final decision/class and provide a thorough reasoning. We measure the success of or system on Agile Modeling nuanced concepts as well as a selection of mainstream image classification sets.

==> old/abstract_v2.tex <==
The Agile Modeling task seeks to enable users to create bespoke classifiers, often with highly nuanced and subjective class definitions. Traditionally, these systems demand substantial human input from the user and/or crowd-annotators in order to achieve accurate classification and may suffer from various biases. In this paper, we introduce Modeling Copilot which seeks to reduce the amount of human input while maintaining high quality by orchestrating a mix of large-language models (LLMs) and vision-language models (VLMs). As part of Modeling Copilot, we propose an Annotator system that is prompted using a concept name and its description, and using LLMs with tool-use, we output a light-weight distilled binary image classifier. We leverage LLM reasoning capabilities to tackle the nuanced nature of subjective image classification tasks. We benchmark our system on nuanced concepts as well as a selection of public image classification sets. We measure the success of our system based on the final distilled binary classification model quality. We show that, while concept-owner feedback is beneficial to the final model quality, Modeling Copilot completely outperforms and eliminates the need for crowd-sourced annotations. In comparison to state-of-the-art zero-shot classification models—including ALIGN, CLIP, CuPL, and VQA models like PaLI—Modeling Copilot Annotator exhibits superior performance. Furthermore, we show that the traditional manual approach of user-provided input is improved by combining with Modeling Copilot.

==> old/abstract_v3.tex <==
From content moderation to wildlife conservation, the number of applications that require models to recognize nuanced or subjective visual concepts is growing. Recently, Agile Modeling proposed a framework to empower any user to quickly bootstrap subjective image classifiers by iteratively labeling positive and negative examples. Although effective, the proposed instantiation of the Agile Modeling is cumbersome; users spend nearly 30 minutes of monotonous, repetitive data labeling to train a single classifier. Drawing on Fiske’s Cognitive Miser theory, we propose a new framework that alleviates human effort by replacing human labeling with natural language interactions – and reducing the total number of interactions required to define a concept by an order of magnitude (from labeling 2,000 images to only 100 with some natural language interactions).  Our framework leverages the recent advances in foundation models, both large language models and vision-language models, to carve out the concept space through conversation, and by automatically labeling training data points.  Most importantly, our framework eliminates the need for crowd-sourced annotations.  Similar to the original Agile Modeling, our framework outputs a light-weight subjective image classifier.  Across 14 subjective concepts and across 3 public image classification datasets, our trained models outperform traditional Agile Modeling. Our system also outperforms state-of-the-art zero-shot classification models like ALIGN, CLIP, CuPL, and large visual question answering models like PaLI. 

==> old/abstract_v4.tex <==

From content moderation to wildlife conservation, the number of applications that require models to recognize nuanced or subjective visual concepts is growing. Traditionally, developing classifiers for such concepts requires substantial manual effort measured in hours, days, or even months to identify and annotate data needed for training. Even with recently proposed Agile Modeling techniques, which enable rapid bootstrapping of image classifiers, users are still required to spend 30 minutes or more of monotonous, repetitive data labeling just to train a single classifier. Drawing on Fiske’s Cognitive Miser theory, we propose a new framework that alleviates manual effort by replacing human labeling with natural language interactions – reducing the total effort required to define a concept by an order of magnitude: from labeling 2,000 images to only 100 plus some natural language interactions. Our framework leverages the recent advances in foundation models, both large language models and vision-language models, to carve out the concept space through conversation and by automatically labeling training data points. Most importantly, our framework eliminates the need for crowd-sourced annotations. Moreover, our framework ultimately produces light-weight classification models that are deployable in cost-sensitive scenarios. Across 14 subjective concepts and across 3 public image classification datasets, our trained models outperform traditional Agile Modeling as well as state-of-the-art zero-shot classification models like ALIGN, CLIP, CuPL, and large visual question answering models like PaLI. 


==> old/intro_v1.tex <==
\section{Introduction} %--------------------------------------------------------
\label{sec:intro}
\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{figures/pali-vs-modeling-copilot.pdf}
    \caption{Visual question answering (VQA) using PaLI-X \cite{chen2023pali} and different prompt with respect to a positive image for the visual concept \texttt{gourmet tuna}. Our Modeling Collaborator Annotator answer is also given for comparison. While VQA models tend to be sensitive the input prompt, our system can reduce that sensitivity through the use of LLM chain-of-thought reasoning capabilities.}
    \label{fig:pali-vs-modeling-copilot}
\end{figure}

Computer vision has primarily focused on recognizing concepts that are objectively agreed upon such as dogs, cats, or cars\cite{deng2009imagenet,lin2014microsoft,kuznetsova2020open} and this is even true for more complex visual classification tasks like fine-grained or compositional (e.g., "red car") recognition. Research on classification of subjective and nuanced concepts is not extensively covered in academic literature and generally involves substantial investments in dataset curation (e.g., emotion recognition, aesthetic classification, content moderation) \cite{khosla2015understanding,connie2017smart,roy2017automated,kiela2020hateful}. The difficulty of this task stems from the nuanced and often ambiguous nature of attributes such as ``creepiness'', ``weirdness'', or ``cuteness''. Practical real-world examples of subjective classification include (a) A content moderator (expert) seeking to remove ``unsafe'' content, where the definition of ``unsafe'' can vary significantly depending on the context, or (b) A food review site aiming to identify ``gourmet tuna'' dishes (as opposed to canned tuna or tuna sandwiches).

% When dealing with subjective image classification, it is crucial to have clear guidelines if crowd annotators are used during the data labeling process.
% Additionally, it is often beneficial to collect multiple annotations per image and use consensus or average scores to minimize individual biases.
Humans possess a remarkable ability to break down complex concepts into more manageable and straightforward components by applying first-order logic\cite{miller1956magical,frege1879begriffsschrift}. For instance, consider a complex concept $\mathcal{X}$. For this concept to be fully understood or realized, elements $\mathcal{Y}$ and $\mathcal{Z}$ are essential and at least one among the elements $\mathcal{A}$, $\mathcal{B}$, or $\mathcal{C}$ must be present. While concept $\mathcal{X}$ may be complex and subjective, $\mathcal{Y}$, $\mathcal{Z}$, $\mathcal{A}$, $\mathcal{B}$, and $\mathcal{C}$ can be simple objective concepts that are easier to quantify. With this in mind, can we (i) leverage LLMs \cite{brown2020gpt3,devlin2018bert,openai2023gpt4} to break down a subjective, nuanced concept into its fundamental logical subcomponents? and (ii) employ LLMs to emulate human-like reasoning in classifying these nuanced concepts?

We deliver Modeling Collaborator; a framework that empowers concept owners to build classifiers by leveraging their expertise. We leverage advancements in LLMs \cite{chowdhery2022palm,anil2023palm2} and VLMs \cite{chen2022pali,chen2023pali,chen2023pali3} to guide people in answering questions about their concepts and automatically generating a classifier for $\mathcal{X}$. For a given image and a concept $\mathcal{X}$, our frameworks employs a supervisor LLM to break down a complex concept into questions that are digestible for a visual question answering (VQA) model \cite{chen2022pali}. This supervisor LLM then asks these questions to the VQA model. Worker LLMs are employed to summarize questions and answers as well as perform various operations to streamline the information flow Finally, the supervisor LLM performs reasoning through chain-of-thought \cite{wei2022chain} to classify an image as positive or negative for $\mathcal{X}$. Additionally, we use our system to autonomously mine data for active learning and distill a light-weight model for each binary classification concept $\mathcal{X}$. We validate the effectiveness of our framework through a set of experiments:
\begin{itemize}
    \item We propose Modeling Collaborator powered by LLMs and VLMs, and demonstrate its ability to quickly build visual classifiers for nuanced concepts.
    \item We compare the quality of our system to traditional Agile Modeling \cite{stretcu2023agile}, where our system replaces both users and/or crowd-raters.

    \item We conduct an ablation study to measure the effectiveness of different components/ideas within our system, and to show how our system effectively addresses the limitations in LLMs and VLMs.
\end{itemize}

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}


